Multi-Static Cell-Free Massive MIMO ISAC: Performance Analysis and Power Allocation

In this work, we consider a cell-free massive multiple-input multiple-output (MIMO) integarted sensing and communications (ISAC) system with maximum-ratio transmission schemes combined with multistatic radar-type sensing. Our focus lies on deriving closed-form expressions for the achievable communications rate and the Cram\'er-Rao lower bound (CRLB), which serve as performance metrics for communications and sensing operations, respectively. The expressions enable us to investigate important operational characteristics of multistatic cell-free massive MIMO-ISAC, including the mutual effects of communications and sensing as well as the advantages stemming from using numerous distributed antenna arrays for each functionality. Furthermore, we optimize the power allocation among the access points to maximize the communications rate while guaranteeing the CRLB constraints and total transmit power budget. Extensive numerical results are presented to validate our theoretical findings and demonstrate the efficiency of the proposed power allocation approach.

==> ASILOMAR24_CFmMIMO_CRLB/Definition.tex <==
% Packages used
\usepackage{amsmath,graphicx}
\usepackage{color}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{empheq}

\usepackage{mathrsfs}
%\usepackage{dutchcal}
\usepackage{hyperref}
%\usepackage{amsthm}
\usepackage{tikz}
%\usepackage[bbgreekl]{mathbbol}
%\DeclareSymbolFontAlphabet{\mathbbm}{bbold}
\usepackage{bm}
\usepackage[english]{babel}
\usepackage{cite}
\usepackage{rotfloat}
\usepackage{mathtools}
\usepackage[font=normalsize,labelfont=bf]{caption}
%\usepackage{breqn}
\usepackage{amsmath}
\usepackage{makecell}
\usepackage{algorithmic}
%\usepackage[ruled, vlined, linesnumbered]{algorithm2e}
\usepackage{multirow}
\usepackage{subfigure}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{multirow}% http://ctan.org/pkg/multirow
\usepackage{hhline}% http://ctan.org/pkg/hhline
\usepackage{stfloats}% <-- added
\usepackage{multicol}
\usepackage{bbm}
\usepackage{cases}
\usepackage[linesnumbered,ruled,lined]{algorithm2e}

\graphicspath{ {Figures/} }
\setlength{\textfloatsep}{0.1cm}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\setlength{\abovecaptionskip}{0.1cm} % Chosen fairly arbitrarily
\newcommand{\eqtext}[1]{\ensuremath{\stackrel{\text{#1}}{=}}}

% transpose, hermitian transpose
\newcommand{\T}{{\scriptscriptstyle\mathsf{T}}}
\renewcommand{\H}{{\scriptscriptstyle\mathsf{H}}}

\newsavebox{\foobox}
\newcommand{\slantbox}[2][.3]
{%
	\mbox
	{%
		\sbox{\foobox}{#2}%
		\hskip\wd\foobox
		\pdfsave
		\pdfsetmatrix{1 0 #1 1}%
		\llap{\usebox{\foobox}}%
		\pdfrestore
	}%
}
\newcommand{\setA}{\mathcal{A}}

\definecolor{kugray5}{RGB}{224,224,224}

\usepackage[normalem]{ulem}
\newcommand\rsout{\bgroup\markoverwith
	{\textcolor{red}{\rule[0.5ex]{2pt}{0.8pt}}}\ULon}

%% ALLOW TO DIVIDE AN ALGORITHM INTO TWO PAGES
\makeatletter
\newenvironment{breakablealgorithm}
{% \begin{breakablealgorithm}
		\begin{center}
			\refstepcounter{algorithm}% New algorithm
			\hrule height.8pt depth0pt \kern2pt% \@fs@pre for \@fs@ruled
			\renewcommand{\caption}[2][\relax]{% Make a new \caption
				{\raggedright\textbf{\ALG@name~\thealgorithm} ##2\par}%
				\ifx\relax##1\relax % #1 is \relax
				\addcontentsline{loa}{algorithm}{\protect\numberline{\thealgorithm}##2}%
				\else % #1 is not \relax
				\addcontentsline{loa}{algorithm}{\protect\numberline{\thealgorithm}##1}%
				\fi
				\kern2pt\hrule\kern2pt
			}
		}{% \end{breakablealgorithm}
		\kern2pt\hrule\relax% \@fs@post for \@fs@ruled
	\end{center}
}
\makeatother

% Color definition
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}

% vector
\newcommand{\myvec}[1]{\ensuremath{\begin{pmatrix}#1\end{pmatrix}}}

% Algorithmic modifications
\makeatletter
\newcommand{\ALOOP}[1]{\ALC@it\algorithmicloop\ #1%
	\begin{ALC@loop}}
	\newcommand{\ENDALOOP}{\end{ALC@loop}\ALC@it\algorithmicendloop}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\algorithmicbreak}{\textbf{break}}
\newcommand{\BREAK}{\STATE \algorithmicbreak}
\makeatother

% Folder of all figures
\usepackage{etoolbox}
\let\mybibitem\bibitem
\renewcommand{\bibitem}[1]{%
	\ifstrequal{#1}{nature}
	{\color{blue}\mybibitem{#1}}
	{\color{black}\mybibitem{#1}}%
}

\graphicspath{ {Figures/} }

% To define the theorems, definitions, remark, lemma, corollary, proof
\newtheorem{definition}{\textbf{Definition}}
\newtheorem{theorem}{\textbf{Theorem}}
\newtheorem{remark}{\textbf{Remark}}
\newtheorem{lemma}{\textbf{Lemma}}
\newtheorem{corollary}{\textbf{Corollary}}
\newtheorem{proof}{Proof}
\renewcommand\theproof{\unskip}
\newcommand{\epr}{\hfill\(\Box\)}

% for 0.1cm and 0.25cm space
\newcommand{\dis}{\hspace{0.1cm}}
\DeclareCaptionLabelSeparator{periodspace}{.\quad}

% for format of Fig. in IEEE
\renewcommand{\figurename}{Fig.}
% to be able to place 2 figure consecutive at the top of page
\captionsetup{font=footnotesize,labelsep=periodspace,singlelinecheck=false}
\captionsetup[sub]{font=footnotesize,singlelinecheck=true}
\addto\captionsenglish{\renewcommand{\figurename}{Fig.}}
% to be able to palce appendices right after conclusion
\interdisplaylinepenalty=2500 

\newcommand\nbthis{\addtocounter{equation}{1}\tag{\theequation}}

% math notations and notations
\newcommand{\norm}[1]{\left\lVert#1\right\rVert} % ||.||
\newcommand{\normshort}[1]{\lVert#1\rVert} % ||.||
\newcommand{\eq}[1]{\begin{align*}#1\end{align*}} % equation
\newcommand{\eqn}[1]{\begin{align}#1\end{align}} % equation
\newcommand{\nt}[1]{\left(#1\right)} % ()
\newcommand{\nv}[1]{\left[#1\right]} % []
\newcommand{\nn}[1]{\left\{#1\right\}} % {}
\newcommand{\abs}[1]{\left|#1\right|} % ||
\newcommand{\absshort}[1]{|#1|} % ||
\newcommand{\nb}{\numberthis}
\newcommand{\tr}[1]{\text{trace}\left(#1\right)} % ||
\newcommand{\vect}[1]{\mathtt{vec}\left(#1\right)} % ||
\newcommand{\trshort}[1]{\text{trace}(#1)} % ||

\newcommand{\detm}[1]{\text{det}\left(#1\right)} % ||
\newcommand{\trsq}[1]{\text{trace}^2\left(#1\right)} % ||
\newcommand{\diag}[1]{\mathtt{diag}\left\{#1\right\}} % ||
\newcommand{\var}[1]{\mathbb{V}\mathtt{ar}\left(#1\right)} % ||
\newcommand{\ds}{\displaystyle}
% real and imag part
\newcommand{\re}[1]{\mathfrak{R}{\left(#1\right)}}
\newcommand{\im}[1]{\mathfrak{I}{\left(#1\right)}}
\allowdisplaybreaks
% Prob, PDF, CDF
%\newcommand{\prob}{\mathbb{P}} 
\newcommand{\cdf}{\mathbf{\textit{F}}} 
\newcommand{\diagtt}{\mathtt{diag}}
\newcommand{\pdf}{\mathbf{\textit{f}}} 
\newcommand{\mean}[1]{\mathbb{E} \left\{#1\right\}}
\newcommand{\meanshort}[1]{\mathbb{E} \{#1\}}

\newcommand{\cov}[1]{\mathbb{C} \left\{#1\right\}}
\newcommand{\meanBig}[1]{\mathbb{E} \Big\{#1\Big\}}
\newcommand{\covBig}[1]{\mathbb{C} \Big\{#1\Big\}}

\usepackage{setspace}
% Problem name
\newcommand{\phybrid}{\left(\mathtt{P}_{\mathtt{hybrid}} \right)}
\newcommand{\pnhybrid}{\left(\mathtt{P-n}_{\mathtt{hybrid}} \right)}
\newcommand{\pnbhybrid}{\left(\var{\mathtt{Pn}}_{\mathtt{hybrid}} \right)}
\newcommand{\ppassive}{\left(\mathtt{P}_{\mathtt{passive}} \right)}
\newcommand{\pactive}{\left(\mathtt{P}_{\mathtt{active}} \right)}
\newcommand{\pnpassive}{\left(\mathtt{P-n}_{\mathtt{passive}} \right)}
\newcommand{\pnuniform}{\left(\mathtt{P-n}_{\mathtt{uniform}} \right)}
\newcommand{\pnhybridLB}{\left(\mathtt{P-n}_{\mathtt{fixed, uni.}} \right)}
\newcommand{\pdyn}{\left(\mathtt{P}_{\mathtt{dyn}} \right)}
\newcommand{\pdyna}{\left(\mathtt{P1}_{\mathtt{dyn}} \right)}
\newcommand{\prob}{\left(\mathtt{P} \right)}
\newcommand{\probn}{\left(\mathtt{Pn} \right)}
% Parameters

% Matrix
\newcommand{\mQ}{{\mathbf{Q}}}
\newcommand{\mR}{{\mathbf{R}}}
\newcommand{\mH}{{\mathbf{H}}} 
\newcommand{\mhsorted}{\underline{\mH}}
\newcommand{\mA}{{\mathbf{A}}}
\newcommand{\mS}{{\mathbf{S}}}
\newcommand{\mW}{{\mathbf{W}}}
\newcommand{\mP}{{\mathbf{P}}}
\newcommand{\mI}{\textbf{\textbf{I}}}
\newcommand{\mT}{{\mathbf{T}}}
\newcommand{\mB}{{\mathbf{B}}}
\newcommand{\mC}{{\mathbf{C}}}
\newcommand{\mD}{{\mathbf{D}}}
\newcommand{\mX}{{\mathbf{X}}}
\newcommand{\mY}{{\mathbf{Y}}}
\newcommand{\mG}{{\mathbf{G}}}
\newcommand{\mF}{{\mathbf{F}}}
\newcommand{\mU}{{\mathbf{U}}}
\newcommand{\mV}{{\mathbf{V}}}
\newcommand{\mE}{{\mathbf{E}}}
\newcommand{\mHr}{{\mathbf{H}}_r} 
\newcommand{\mHt}{{\mathbf{H}}_t} 
\newcommand{\mIr}{{\mathbf{I}}_{N_r}}
\newcommand{\mZ}{{\mathbf{Z}}}
\newcommand{\mK}{{\mathbf{K}}}
\newcommand{\mN}{{\mathbf{N}}}
\newcommand{\mM}{{\mathbf{M}}}
\newcommand{\mRn}{{\mR_{\mathtt{n}}}}
\newcommand{\mRninv}{\mR_{\mathtt{n}}^{-1}}
\newcommand{\mJ}{{\mathbf{J}}}
\newcommand{\Na}{N_{\mathtt{A}}}
\def\mathbi#1{\textbf{\em #1}}

% max value
\newcommand{\Xm}{X_{max}} 
\newcommand{\Am}{A_{max}} 
\newcommand{\Bm}{B_{min}} 


%% Set
\newcommand{\setC}{\mathbb{C}} 
\newcommand{\setR}{\mathbb{R}}
%\newcommand{\setA}{\mathcal{A}} 
\newcommand{\setD}{\mathcal{D}} 
\newcommand{\setANt}{\setA^{N_t}} 
\newcommand{\setAtld}{\tilde{\setA}^{N_t}}
\newcommand{\setN}{\mathbb{N}}

%% List
\newcommand{\ltabu}{\mathcal{L}}
\newcommand{\leta}{\mathcal{L}_{\eta}}
\newcommand{\lphi}{\mathcal{L}_{\phi}}

%% Probability
\newcommand{\Pe}{\mathcal{P}}
\newcommand{\Pne}{\var{\mathcal{P}}}

%% Vector
\newcommand{\vxb}{{\mathbf{x}}^{\star}}
\newcommand{\vc}{{\mathbf{c}}}
\newcommand{\vci}{{\mathbf{c}}_{\nn{1}}}
\newcommand{\ve}{{\mathbf{e}}} 
\newcommand{\vs}{{\mathbf{s}}}
\newcommand{\vx}{{\mathbf{x}}}
\newcommand{\vy}{{\mathbf{y}}}
\newcommand{\vr}{{\mathbf{r}}}
\newcommand{\vqn}{{\mathbf{q}}^T_n}
\newcommand{\vpnT}{{\mathbf{p}}^T_n}
%\newcommand{\vpnT}{{\mathbf{r}}^T_n}
\newcommand{\vpd}{{\mathbf{p}}_d}
\newcommand{\vrdc}{\check{{\mathbf{r}}}_d}
\newcommand{\vhdc}{\check{{\mathbf{h}}}_d}
\newcommand{\vhc}{\check{{\mathbf{h}}}}
\newcommand{\vrd}{{\mathbf{r}}_d}
\newcommand{\vrds}{{\mathbf{r}}_{d^{\star}}}
\newcommand{\vpn}{{\mathbf{p}}_n}
\newcommand{\vv}{{\mathbf{v}}}
\newcommand{\vn}{{\mathbf{n}}}
\newcommand{\vu}{{\mathbf{u}}}
\newcommand{\vz}{{\mathbf{z}}} 
\newcommand{\vh}{{\mathbf{h}}} 
\newcommand{\vhd}{{\mathbf{h}}_d}
\newcommand{\vq}{{\mathbf{q}}}
\newcommand{\vb}{{\mathbf{b}}}
\newcommand{\vw}{{\mathbf{w}}}
\newcommand{\va}{{\mathbf{a}}}
\newcommand{\vd}{{\mathbf{d}}}
\newcommand{\vt}{{\mathbf{t}}}
\newcommand{\vg}{{\mathbf{g}}}
\newcommand{\vp}{{\mathbf{p}}}
\newcommand{\vi}{{\mathbf{i}}}

%% Elements of vectors/matrice
\newcommand{\zbn}{\var{z}_n}
\newcommand{\rni}{r_{n,i}}
\newcommand{\rnj}{r_{n,j}}
\newcommand{\pnj}{p_{n,j}}
\newcommand{\qni}{q_{n,i}}
\newcommand{\qnj}{q_{n,j}}

%% Other notations
\newcommand{\dx}{\Delta{\mathbf{x}}}

\newcommand{\mpeta}[1]{\phi_{#1} (\vx)} % Metric
\newcommand{\mpetai}[1]{\phi_{#1} (\vx_{[i]})} % Metric

\newcommand{\smt}{\sigma_t^2} % Power
\newcommand{\smv}{\sigma_v^2} % Power
\newcommand{\smn}{\sigma_n^2} % Power

\newcommand{\pbar}{\var{\Phi}}
\newcommand{\ptilde}{\tilde{\Phi}}

\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bUpsilon}{\boldsymbol{\Upsilon}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}

\newcommand{\Pa}{P_{\mathtt{a}}} 
\newcommand{\Pamax}{P_{\mathtt{a}}^{\mathtt{max}}}
\newcommand{\Pap}{P_{\mathtt{AP}}}
\newcommand{\amn}{\alpha_{mn}}
\newcommand{\amns}{\alpha_{mn}^{\star}}
\newcommand{\vphi}{\boldsymbol{\varphi}}
\newcommand{\vmu}{\boldsymbol{\mu}}
\newcommand{\vgamma}{\var{\boldsymbol{\gamma}}}
\newcommand{\veta}{\var{\boldsymbol{\eta}}}
\newcommand{\vf}{\mathbf{f}}
\newcommand{\vnu}{\boldsymbol{\nu}}
\newcommand{\vomega}{\boldsymbol{\omega}}
\newcommand{\valpha}{\boldsymbol{\alpha}}
%\newcommand{\mSigma}{\boldsymbol{\Sigma}}




\def\redmark{\textcolor{red}}
\def\argmin{\mathop{\mathtt{argmin}}}
\def\argmax{\mathop{\mathtt{argmax}}}
%\def\diag{\mathop{\mathtt{diag}}}
\def\inf{\mathop{\mathtt{in}}}
\def\outf{\mathop{\mathtt{out}}}
\def\trace{\mathop{\text{tr}}}
%\def\span{\mathop{\mathtt{span}}}
\def\dim{\mathop{\mathtt{dim}}}
\def\Re{\mathop{\mathtt{Re}}}
\def\Im{\mathop{\mathtt{Im}}}
\def\redmark{\textcolor{red}}

\newcommand{\Ei}{{\mathtt{Ei}}}

\def\bDelta{{\pmb{\Delta}}} \def\bdelta{{\pmb{\delta}}}
\def\bSigma{{\pmb{\Sigma}}} \def\bsigma{{\pmb{\sigma}}}
\def\bPhi{{\pmb{\Phi}}} \def\bphi{{\pmb{\phi}}}
\def\bGamma{{\pmb{\Gamma}}} \def\bgamma{{\pmb{\gamma}}}
\def\bOmega{{\pmb{\Omega}}} \def\bomega{{\pmb{\omega}}}
\def\bTheta{{\pmb{\Theta}}} \def\btheta{{\pmb{\theta}}}
\def\bepsilon{{\pmb{\epsilon}}} \def\bPsi{{\pmb{\Psi}}}
\def\obH{\overline{\bH}}\def\obw{\overline{\bw}} \def\obz{\overline{\bz}}\def\bmu{{\pmb{\mu}}}
\def\b0{{\pmb{0}}}\def\bLambda{{\pmb{\Lambda}}} \def\oc{\overline{\bc}}

\newcommand{\Frf}{\mF_\mathtt{RF}}
\newcommand{\Fopt}{\mF_{\text{opt}}}

\newcommand{\Frft}{\tilde{\mF}_\mathtt{RF}}
\newcommand{\Fbb}{\mF_\mathtt{BB}}
\newcommand{\fbb}{\vf_\mathtt{BB}}

\newcommand{\Wrf}{\bW_\mathtt{RF}}
\newcommand{\Wbb}{\bW_\mathtt{BB}}
\newcommand{\Nrf}{N_{\text{RF}}} 
\newcommand{\Nr}{N_\mathtt{r}}
\newcommand{\Nt}{N_\mathtt{t}} 
\newcommand{\Mr}{M_\mathtt{r}}
\newcommand{\Mt}{M_\mathtt{t}} 
\newcommand{\Nu}{N_\mathtt{u}}
\newcommand{\Ntn}{N_{\text{t},n}} 
\newcommand{\Ntnt}{\tilde{N}_{\text{t},n}} 
\newcommand{\Ns}{N_\mathtt{s}}
\newcommand{\Nrh}{N_\mathtt{rh}}
\newcommand{\Nrv}{N_\mathtt{rv}}
\newcommand{\Nth}{N_\mathtt{th}}
\newcommand{\Ntv}{N_\mathtt{tv}}

\newcommand{\Nrhn}{N_{\text{r},n}^\mathtt{h}}
\newcommand{\Nrvn}{N_{\text{r},n}^\mathtt{v}}
\newcommand{\Nthn}{N_{\text{t},n}^\mathtt{h}}
\newcommand{\Ntvn}{N_{\text{t},n}^\mathtt{v}}
\newcommand{\Nms}{N_{\text{MS}}} 


\newcommand{\Nrfr}{N_{\text{RF,r}}}
\newcommand{\Nrft}{N_{\text{RF,t}}}
\newcommand{\Mnr}{M_{n,\text{r}}}
\newcommand{\Mnt}{M_{n,\text{t}}}
\newcommand{\ar}{\va_\mathtt{r}} 
\newcommand{\at}{\va_\mathtt{t}} 
\newcommand{\arh}{\va_\mathtt{r,h}} 
\newcommand{\arv}{\va_\mathtt{r,v}} 
\newcommand{\ah}{\va_\mathtt{h}} 
\newcommand{\av}{\va_\mathtt{v}}
\newcommand{\art}{\tilde{\va}_\mathtt{r}} 
\newcommand{\att}{\tilde{\va}_\mathtt{t}} 
\newcommand{\atht}{\tilde{\va}_\mathtt{t,h}} 
\newcommand{\atvt}{\tilde{\va}_\mathtt{t,v}}
\newcommand{\dat}{{\dot{\va}_\mathtt{t}}} 
\newcommand{\ih}{i_\mathtt{h}} 
\newcommand{\iv}{i_\mathtt{v}} 
\newcommand{\dath}{\dot{\va}_\mathtt{t,h}} 
\newcommand{\datv}{\dot{\va}_\mathtt{t,v}}

\newcommand{\Afull}{\mathcal{A}_{\text{full}}}
\newcommand{\Asub}{\mathcal{A}_{\text{sub}}}

\newcommand{\setK}{\mathcal{K}}
\newcommand{\setT}{\mathcal{T}}
\newcommand{\setJ}{\mathcal{J}}
\newcommand{\setMt}{\mathcal{M}_{\mathtt{t}}}
\newcommand{\setMr}{\mathcal{M}_{\mathtt{r}}}
\newcommand{\setTheta}{\bm{\Theta_{\text{d}}}}
\newcommand{\Pbs}{P_{\text{BS}}}
\newcommand{\fronorm}[1]{\left\lVert#1\right\rVert_{\mathcal{F}}} % ||.||
\newcommand{\sigmac}{\sigma_{\mathtt{c}}^2}
\newcommand{\sigmas}{\sigma_{\mathtt{s}}^2}
\newcommand{\noiseu}{\sigma_{\mathtt{u}}^2}
\newcommand{\noiser}{\sigma_{\mathtt{r}}^2}
\newcommand{\noiserb}{\bar{\sigma}_{\mathtt{r}}^2}
\newcommand{\noise}{\sigma^2}
\newcommand{\Pt}{P_{\mathtt{t}}}

\newcommand{\Jtt}{J_{\theta \theta}}
\newcommand{\Jtp}{J_{\theta \phi}}
\newcommand{\Jta}{\mJ_{\theta \bar{\bm{\alpha}}}}
\newcommand{\Jpp}{J_{\phi \phi}}
\newcommand{\Jpa}{\mJ_{\phi \bar{\bm{\alpha}}}}
\newcommand{\Jaa}{\mJ_{\bar{\bm{\alpha}}\bar{\bm{\alpha}}}}
\newcommand{\Jpat}{\tilde{J}_{\phi \bar{\bm{\alpha}}}}


\newcommand{\xibf}{\bm{\xi}_{\mathtt{bf}}}
\newcommand{\lambdabf}{{\lambda_{\mathtt{bf}}}} 
\newcommand{\zetabf}{{\bm{\zeta}_{\mathtt{bf}}}}
\newcommand{\adotphi}{\dot{\va}_{\phi}}
\newcommand{\adottheta}{\dot{\va}_{\theta}}
\newcommand{\bdotphi}{\dot{\vb}_{\phi}}
\newcommand{\bdottheta}{\dot{\vb}_{\theta}}


